Adversarial Examples: Attacks and Defenses for Deep Learning

With rapid progress and significant successes in a wide spectrum of applications, deep learning is being applied in many safety-critical environments. However, deep neural networks have been recently found vulnerable to well-designed input samples, called adversarial examples. Adversarial examples are imperceptible to human but can easily fool deep neural networks in the testing/deploying stage. The vulnerability to adversarial examples becomes one of the major risks for applying deep neural networks in safety-critical environments. Therefore, attacks and defenses on adversarial examples draw great attention. In this paper, we review recent findings on adversarial examples for deep neural networks, summarize the methods for generating adversarial examples, and propose a taxonomy of these methods. Under the taxonomy, applications for adversarial examples are investigated. We further elaborate on countermeasures for adversarial examples and explore the challenges and the potential solutions.

==> adv.tex <==
In this section, we will introduce attack approaches and countermeasures for adversarial examples and try to answer the following questions:

1) What are adversarial examples? 2) How to generate adversarial examples? 3) Why can adversarial examples successfully fool deep neural networks? 4) What are the existing countermeasures? 5) What can deep learning researchers learn from adversarial examples?

\subsection{Overview}
Using a trained model by a third party, a user inputs testing data samples to get prediction. \advs are original input data with small perturbations, often barely recognizable by human. However, such perturbations misguide the model to classify the perturbed data into another incorrect category. Typically, adversarial examples are generated against a supervised classification model. For most of the existing attack methods, adversarial examples can easily be generalized from binary classification model to multi-class classification model.

To our best knowledge, there are only a few research projects on other kinds of machine learning problems, such as semi-supervised learning (\cite{miyato2015distributional}), generative models (\cite{kos2017adversarial}), and reinforcement learning (\cite{huang2017adversarial}). 

For a multi-classification problem, an adversary tries to misguide the classifier to predict a wrong label of a perturbed data sample. In the meanwhile, the perturbation should be constraint in a small scale that can hardly be recognized by human. Hence, given a trained deep learning model $f$, an original input data sample $x$, generating an adversarial example $x'$ can be described as a box-constrained optimization problem:
\begin{align*} 
% \label{eq:general}
&\min_{x'} && \|x'-x\| \\
& s.t. && f(x') =l', \\
& && f(x) = l, \\
& && l \neq l', \\
& && x' \in [0, 1],
\end{align*}
where $l$ and $l'$ are the output label of $x$ and $x'$. Let $r = x' - x$ be the magnitude of perturbation added on $x$. Some adversaries consider that if $\|r\|\leq \delta$, the perturbation is small enough and not noticeable to human. Therefore, the optimization objective can be the distance of targeted prediction score and the original prediction score.  
% In some work, the perturbation within a certain threshold is considered good enough to be unrecognizable for human. 
Thus, another variant for generating adversarial example is:
\begin{align*} 
% \label{eq:variant}
\min_{x'} \quad & \|f(x')-l'\| \\
s.t. \quad \|x-x'\| &  \leq \delta, \\
f(x) & = l, \\
l & \neq l'
\end{align*}



\subsection{Other Application Attacks}
\subsubsection{Facial Biometric System}
Sharif \etal conducted a physical attack on facial biometric system~\cite{sharif2016accessorize}.


NO Need to Worry about Adversarial Examples in Object Detection in Autonomous Vehicles~\cite{lu2017no}.

\subsubsection{Speech Recognition System}


==> revision.tex <==
Firstly, we would like to thank all reviewers and editors for your careful consideration of this paper, your helpful comments, and your valuable time spent reviewing our work. We hope that the explanations below address key issues by the reviewers. We summarize our changes (in red) based on reviewers' comments.

\subsection{Reviewer 1}
\begin{itemize}
    \item Page 4, line 37. I would say the datasets are standard DL benchmarks, instead of general dataset. Each dataset is only for one specific task.\\
    \textcolor{red}{We use ``standard dataset'' to refer these datasets.}
    \item In section 4, the authors listed existing approach on adversarial attacks. I would suggest a table joining the methods and taxonomy. In other words, a table specifying which category a method falls into would be very helpful.\\
    \textcolor{red}{We redraw Table~\ref{tab:taxonomy} to put all the methods/papers in each dimension. We also classify them into three main categories.}
    \item Page 11 line 17, it is not clear to me what is the perturbation on groundtruth. Is it about setting label to a nearby class for image classification?\\
    \textcolor{red}{We rewrite the ground-truth attack in Section~\ref{sec:method} to make it clearer.}
    \item The organization of Section VII.B can be improved. The reasons are not well taxonomized. E.g. the related works can be categorized based on the reasons, like covariate shift, coverage of test case.\\
    \textcolor{red}{We categorize the existence of adversarial examples into three main assumptions: data incompletion, model capability, and no robust model.}
    \item Regarding the benchmarks, I would suggest add the NIPS competition on defense and attack.\\
    \textcolor{red}{We discuss the NIPS competition on both (targeted/non-targeted) attack and defense in Section~\ref{sec:analysis_evaluation}.}
    \item \textcolor{red}{We also would like to thank the reviewer for other comments (\eg, notation abuse, grammar errors, and typos). They are corrected in the current version.}
\end{itemize}

\subsection{Reviewer 2}
\begin{itemize}
    \item I think this is a good review about the the attacks and defenses of deep learning with adversarial examples draw great attention. It is suggested to be accepted. \\
    \textcolor{red}{We would like to thank you for your comments.}
\end{itemize}

\subsection{Reviewer 3}
\begin{itemize}
    \item Some concepts in the background selection, such as CNNs, RNNs, dropout, activation functions, should be omitted or replaced by concepts related to the field of attacks and defenses for deep learning.\\
    \textcolor{red}{We remove the basic concepts of deep learning.}
    \item Article structure problem: `an instance of adversarial examples for image classification task' isn't suitable for introduction selection. \\ 
    \textcolor{red}{We move the instance of adversarial examples to the background section.}
    \item The axis of adversarial examples taxonomy should be more hierarchical, for example, perturbation scope, perturbation limitation and perturbation measurement belong to perturbation.\\
    \textcolor{red}{We reconstruct Table II and summarize the categories into three main topics: threat model, perturbation, and benchmark.}
    \item When introducing the methods for generating adversarial examples, you should explain the relationship between method and taxonomy, and use the table 3 as a summary.\\
    \textcolor{red}{We join the method and taxonomy in Table~\ref{tab:taxonomy}. We discuss the relationship between method and taxonomy in Section~\ref{sec:taxonomy}.}
    \item In the summary of applications for adversarial examples (table 3), the table should add an item of the result of each application to explicitly show the performance, for example, the accuracy decrease after adversarial example attacks. \\
    \textcolor{red}{It is hard to compare the performance due to the different benchmarks used (\ie, victim models, datasets, and applications). For example, in the image classification task, six different datasets are used to evaluate the attacks (Table~\ref{tab:taxonomy}). We also believe the performance degradation is just one of the results of adversarial attacks. Adversarial examples also illustrate the inherent vulnerability and semantic incorrectness of deep learning.}
    \item In the description of FGSM algorithm (Page 6), sentences such as 11This method won NIPS 2017 targeted and non-targeted adversarial attacks competition'' is inappropriate in a paper, which seems to have a preference for it. \\ 
    \textcolor{red}{We remove this description in the paper.}
\end{itemize}

\subsection{Reviewer 5}
\begin{itemize}
    \item In this paper, the authors provide a taxonomy for the most relevant types of Adversarial Attacks and Defenses. Although the authors' effort to summarize such a vast subject in a single manuscript is praiseworthy, I do not unfortunately see any scientific research in the manuscript. I think that the type of work that has been done would be better suited for a review article rather than a research paper. Therefore, I encourage submission to a different journal. \\
    \textcolor{red}{We hope this comprehensive survey of emerging topics can contribute to the community with systematic blueprints and guidelines, promote this important research topic, and facilitate junior researchers with well-thought taxonomies and a comprehensive collection of references.}
\end{itemize}
